FOReCAst: The Future Outcome Reasoning and Confidence Assessment Benchmark

Forecasting is an important task in many domains, such as technology and economics. However existing forecasting benchmarks largely lack comprehensive confidence assessment, focus on limited question types, and often consist of artificial questions that do not align with real-world human forecasting needs. To address these gaps, we introduce FOReCAst (Future Outcome Reasoning and Confidence Assessment), a benchmark that evaluates models' ability to make predictions and their confidence in them. FOReCAst spans diverse forecasting scenarios involving Boolean questions, timeframe prediction, and quantity estimation, enabling a comprehensive evaluation of both prediction accuracy and confidence calibration for real-world applications.

==> tables/dataset_distribution.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Question Type}   & \textbf{Number of Questions} \\ \hline
Binary                   &                               \\ \hline
Temporal                 &                               \\ \hline
Quantitative             &                               \\ \hline
\end{tabular}
\caption{Distribution of questions in the \textsc{FOReCAst} dataset by question type.}
\label{tab:forecast_types}
\end{table}

==> tables/dataset_domain_stats.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Domain}       & \textbf{Number of Questions} \\ \hline
Technology            &                               \\ \hline
Health                &                               \\ \hline
Geopolitics           &                               \\ \hline
Economics             &                               \\ \hline
Other                 &                               \\ \hline
\end{tabular}
\caption{Distribution of questions in the \textsc{FOReCAst} dataset by domain.}
\label{tab:forecast_domains}
\end{table}

==> tables/finding_1_result_binary.tex <==
% \begin{table}[ht]
% \centering
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% Model & N & Accuracy ($\uparrow$) & F1 ($\uparrow$) & Brier ($\downarrow$) \\
% \midrule
% GPT2              & 401 & 0.58 & 0.37 & 0.42 \\
% GPT2-XL           & 401 & 0.67 & 0.32 & 0.45 \\
% Pythia-14m        & 343 & 0.59 & 0.14 & 0.62 \\
% Pythia-160m       & 343 & 0.61 & 0.26 & 0.53 \\
% Pythia-2.8b       & 343 & 0.55 & 0.39 & 0.44 \\
% Bloom-560m        & 263 & 0.49 & 0.41 & 0.45 \\
% Bloom-7b1         & 263 & 0.64 & 0.33 & 0.32 \\
% Llama-7b          & 226 & 0.57 & 0.34 & 0.52 \\
% OLMo-1B           & 188 & 0.23 & 0.16 & 0.75 \\
% OLMo-7B           & 188 & 0.21 & 0.17 & 0.82 \\
% OLMo-7B-Instruct  & 188 & 0.65 & 0.14 & 0.38 \\
% OLMo-2-7B         & 145 & 0.51 & 0.24 & 0.44 \\
% OLMo-2-7B-Instruct & 145 & 0.59 & 0.30 & 0.41 \\
% \bottomrule
% \end{tabular}%
% % }
% \caption{Performance of forecasting models on Boolean questions in \textsc{FOReCAst}. Reported metrics include the number of evaluated questions (N), accuracy, F1 score (both higher is better), and the Brier score (lower is better).}
% \label{tab:binary_forecasting}
% \end{table}


\begin{table}[ht]
\centering
\caption{Performance of forecasting models on Boolean questions in \textsc{FOReCAst}. Reported metrics include the number of evaluated questions (N), accuracy, F1 score (both higher is better), and the Brier score (lower is better).}
\footnotesize % smaller font
\begin{tabular}{lcccc}
\toprule
Model & N & Accuracy ($\uparrow$) & F1 ($\uparrow$) & Brier ($\downarrow$) \\
\midrule
GPT2              & 401 & 0.58 & 0.37 & 0.42 \\
GPT2-XL           & 401 & 0.67 & 0.32 & 0.45 \\
Pythia-14m        & 343 & 0.59 & 0.14 & 0.62 \\
Pythia-160m       & 343 & 0.61 & 0.26 & 0.53 \\
Pythia-2.8b       & 343 & 0.55 & 0.39 & 0.44 \\
Bloom-560m        & 263 & 0.49 & 0.41 & 0.45 \\
Bloom-7b1         & 263 & 0.64 & 0.33 & 0.32 \\
Llama-7b          & 226 & 0.57 & 0.34 & 0.52 \\
OLMo-1B           & 188 & 0.23 & 0.16 & 0.75 \\
OLMo-7B           & 188 & 0.21 & 0.17 & 0.82 \\
OLMo-7B-Inst  & 188 & 0.65 & 0.14 & 0.38 \\
OLMo-2-7B         & 145 & 0.51 & 0.24 & 0.44 \\
OLMo-2-7B-Inst & 145 & 0.59 & 0.30 & 0.41 \\
\bottomrule
\end{tabular}%

\label{tab:binary_forecasting}
\end{table}


==> tables/finding_1_result_quantity.tex <==
% \begin{table}[ht]
% \centering
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% Model & N & APE ($\downarrow$) & MAE ($\downarrow$) & CRPS ($\downarrow$) \\
% \midrule
% GPT2              & 81 & 0.23 & 0.87 & 0.86 \\
% GPT2-XL           & 81 & 0.03 & 0.75 & 0.72 \\
% Pythia-14m        & 77 & 0.17 & 0.88 & 0.85 \\
% Pythia-160m       & 77 & 0.03 & 0.78 & 0.76 \\
% Pythia-2.8b       & 77 & 0.07 & 0.81 & 0.79 \\
% Bloom-560m        & 43 & 0.05 & 0.73 & 0.71 \\
% Bloom-7b1         & 43 & 0.06 & 0.75 & 0.72 \\
% Llama-7b          & 32 & 0.06 & 0.64 & 0.61 \\
% OLMo-1B           & 23 & 0.21 & 0.79 & 0.76 \\
% OLMo-7B           & 23 & 0.22 & 0.84 & 0.82 \\
% OLMo-7B-Instruct  & 23 & 0.24 & 0.80 & 0.77 \\
% OLMo-2-7B         & 20 & 0.02 & 0.65 & 0.62 \\
% OLMo-2-7B-Instruct & 20 & 0.09 & 0.60 & 0.57 \\
% \bottomrule
% \end{tabular}%
% % }
% \caption{Performance of forecasting models on Quantity Estimation tasks in \textsc{FOReCAst}. Metrics include the number of evaluated questions (N), normalized absolute percentage error (APE), mean absolute error (MAE), and Continuous Ranked Probability Score (CRPS), where lower values are better.}
% \label{tab:quantity_estimation}
% \end{table}


\begin{table}[ht]
\centering
\scriptsize
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Model & N & APE ($\downarrow$) & MAE ($\downarrow$) & CRPS ($\downarrow$) \\
\midrule
GPT2              & 81 & 0.23 & 0.87 & 0.86 \\
GPT2-XL           & 81 & 0.03 & 0.75 & 0.72 \\
Pythia-14m        & 77 & 0.17 & 0.88 & 0.85 \\
Pythia-160m       & 77 & 0.03 & 0.78 & 0.76 \\
Pythia-2.8b       & 77 & 0.07 & 0.81 & 0.79 \\
Bloom-560m        & 43 & 0.05 & 0.73 & 0.71 \\
Bloom-7b1         & 43 & 0.06 & 0.75 & 0.72 \\
Llama-7b          & 32 & 0.06 & 0.64 & 0.61 \\
OLMo-1B           & 23 & 0.21 & 0.79 & 0.76 \\
OLMo-7B           & 23 & 0.22 & 0.84 & 0.82 \\
OLMo-7B-Instruct  & 23 & 0.24 & 0.80 & 0.77 \\
OLMo-2-7B         & 20 & 0.02 & 0.65 & 0.62 \\
OLMo-2-7B-Instruct & 20 & 0.09 & 0.60 & 0.57 \\
\bottomrule
\end{tabular}%
% }
\caption{Performance of forecasting models on Quantity Estimation tasks in \textsc{FOReCAst}. Metrics include the number of evaluated questions (N), normalized absolute percentage error (APE), mean absolute error (MAE), and Continuous Ranked Probability Score (CRPS), where lower values are better.}
\label{tab:quantity_estimation}
\end{table}

==> tables/finding_1_result_timeframe.tex <==
% \begin{table}[ht]
% \centering
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lccc}
% \toprule
% Model & N & ADE ($\downarrow$) & CRPS ($\downarrow$) \\
% \midrule
% GPT2              & 26 & 0.99 & 0.99 \\
% GPT2-XL           & 26 & 1.00 & 1.00 \\
% Pythia-14m        & 25 & 1.00 & 1.00 \\
% Pythia-160m       & 25 & 1.00 & 1.00 \\
% Pythia-2.8b       & 25 & 0.97 & 0.96 \\
% Bloom-560m        & 12 & 1.00 & 1.00 \\
% Bloom-7b1         & 12 & 1.00 & 1.00 \\
% Llama-7b          & 10 & 0.98 & 0.98 \\
% OLMo-1B           & 6  & 1.00 & 1.00 \\
% OLMo-7B           & 6  & 1.00 & 1.00 \\
% OLMo-7B-Instruct  & 6  & 1.00 & 1.00 \\
% OLMo-2-7B         & 4  & 1.00 & 1.00 \\
% OLMo-2-7B-Instruct & 4  & 0.87 & 0.82 \\
% \bottomrule
% \end{tabular}%
% % }
% \caption{Performance of forecasting models on Timeframe Prediction tasks in \textsc{FOReCAst}. Metrics include the number of evaluated questions (N), the normalized absolute days error (ADE), and the Continuous Ranked Probability Score (CRPS), where lower values indicate better performance.}
% \label{tab:timeframe_prediction}
% \end{table}

\begin{table}[ht]
\centering
\scriptsize
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
Model & N & ADE ($\downarrow$) & CRPS ($\downarrow$) \\
\midrule
GPT2              & 26 & 0.99 & 0.99 \\
GPT2-XL           & 26 & 1.00 & 1.00 \\
Pythia-14m        & 25 & 1.00 & 1.00 \\
Pythia-160m       & 25 & 1.00 & 1.00 \\
Pythia-2.8b       & 25 & 0.97 & 0.96 \\
Bloom-560m        & 12 & 1.00 & 1.00 \\
Bloom-7b1         & 12 & 1.00 & 1.00 \\
Llama-7b          & 10 & 0.98 & 0.98 \\
OLMo-1B           & 6  & 1.00 & 1.00 \\
OLMo-7B           & 6  & 1.00 & 1.00 \\
OLMo-7B-Instruct  & 6  & 1.00 & 1.00 \\
OLMo-2-7B         & 4  & 1.00 & 1.00 \\
OLMo-2-7B-Instruct & 4  & 0.87 & 0.82 \\
\bottomrule
\end{tabular}%
% }
\caption{Performance of forecasting models on Quantity Estimation and Timeframe Prediction tasks in \textsc{FOReCAst}. Metrics include the number of evaluated questions (N), normalized absolute percentage error (APE), mean absolute error (MAE), absolute days error (ADE), and Continuous Ranked Probability Score (CRPS), where lower values indicate better performance.}
\label{tab:timeframe_prediction}
\end{table}
